InstaHide's Sample Complexity When Mixing Two Private Images

Training neural networks usually require large numbers of sensitive training data, and how to protect the privacy of training data has thus become a critical topic in deep learning research. InstaHide is a state-of-the-art scheme to protect training data privacy with only minor effects on test accuracy, and its security has become a salient question. In this paper, we systematically study recent attacks on InstaHide and present a unified framework to understand and analyze these attacks. We find that existing attacks either do not have a provable guarantee or can only recover a single private image. On the current InstaHide challenge setup, where each InstaHide image is a mixture of two private images, we present a new algorithm to recover all the private images with a provable guarantee and optimal sample complexity. In addition, we also provide a computational hardness result on retrieving all InstaHide images. Our results demonstrate that InstaHide is not information-theoretically secure but computationally secure in the worst case, even when mixing two private images.

==> checklist.tex <==
\section*{Checklist}




 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> gradient.tex <==
\section{Gradient attack from batch is somehow like Mixup}
\subsection{One Hidden Layer}
We consider a one-hidden layer ReLU activated neural network with $m$ neurons in the hidden layer:
\begin{align*}
    f(x) = a^\top \phi(W x )
\end{align*}
where $a\in \R^m$ and $W \in \R^{m \times d}$.
We define objective function $L$ as follows:
\begin{align*}
    L(W) = \frac{1}{2} \sum_{i=1}^n (y_i - f(W,x_i,a))^2
\end{align*}
We can compute the gradient of $L$ in terms of $w_r$
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = \sum_{i=1}^n ( f(W,x_i,a) -y_i ) a_r x_i {\bf 1}_{ \langle w_r, x_i \rangle }
\end{align*}
Let $\wt{x} = \frac{1}{n} \sum_{i=1}^n x_i$,
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = ( f(W, \wt{x}, a) - y ) a_r \wt{x} {\bf 1}_{\langle w_r, \wt{x} \rangle}
\end{align*}
Another version
\begin{align*}
    \frac{ \partial L(W) }{ \partial w_r } = \sum_{i=1}^n ( f(W, x_i, a) - y_i ) \cdot \Big( a_r \wt{x} {\bf 1}_{\langle w_r, \wt{x} \rangle} \Big)
\end{align*}


\subsection{Two Hidden Layers}

Suppose $a \in \R^m$, $V \in \R^{m \times d}, W \in \R^{m \times m}$. The neural network is defined as $f : \R^d \rightarrow \R$, here we slightly deviate from the standard setting and assume the input dimension is $m$, in order to capture the general setting.
\begin{align*}
f(x) = a^{\top} \phi( W \phi ( V x ) )
\end{align*}
Consider the mean square loss
\begin{align*}
L(W, V, a) = \frac{1}{2} \sum_{i=1}^n | f(x_i) - y_i |^2
\end{align*}
The gradient with respect to $W$ is
\begin{align*}
\frac{ \partial L(W, V, a)}{ \partial W } = \sum_{i=1}^{n}(f(x_i) - y_i)  \underbrace{ \diag\{\phi'(W \phi(Vx_i))\} }_{ m \times m }\underbrace{ a }_{m \times 1}  \underbrace{ \phi(Vx_i)^{\top} }_{1 \times m}  
\end{align*}
and the gradient with respect to $V$ is
\begin{align*}
\frac{ \partial L(W, V, a)}{ \partial V } = \sum_{i=1}^{n}(f(x_i) - y_i)\underbrace{\diag\{ \phi'(Vx_i)\}}_{m \times m} \underbrace{W^{\top}}_{m \times m}  \underbrace{\diag\{\phi'(W \phi(Vx_i))\}}_{m \times m} \underbrace{a}_{m \times 1}    \underbrace{x_i^{\top}}_{1 \times d} 
\end{align*}

\subsection{The multi-layers case}


The following multiple layer neural network definition should be found in \cite{als19_dnn}.

Consider a $L$ layer neural network with one vector $a\in \R^{m_L}$ and $L$ matrices $W_L \in \R^{m_L \times m_{L-1}}$, $\cdots$, $W_2 \in \R^{m_2 \times m_1}$ and $W_1 \in \R^{m_1 \times m_0}$. Let $m_0 = d$.
In order to write gradient in an elegant way, we define some artificial variables as follows
\begin{align}\label{eq:def_g_h}
g_{i,1} = & ~ W_1 x_i, && h_{i,1} = \phi(W_1 x_i), && \in \R^{m_1} && \forall i \in [n]\notag\\
g_{i,\ell} = & ~ W_{\ell} h_{i,\ell-1}, && h_{i,\ell} = \phi( W_{\ell} h_{i,\ell-1} ), && \in \R^{m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \\
D_{i, 1} = & ~ \text{diag} \big(\phi'(W_1 x_i )\big), && && \in \R^{m_1 \times m_1} && \forall i \in [n] \notag\\
D_{i, \ell} = & ~ \text{diag} \big(\phi'(W_{\ell} h_{i, \ell-1})\big), && && \in \R^{m_{\ell} \times m_{\ell}} && \forall i \in [n], \forall \ell \in \{2,3,\cdots,L\} \notag
\end{align}
where $\phi(\cdot)$ is the activation function and $\phi'(\cdot)$ is the derivative of activation function. 



Let $f : \R^{m_0} \rightarrow \R$ denote neural network function: 
\begin{align*}
    f(W,x) = a^\top \phi( W_L ( \phi ( \cdots \phi(W_1 x ) ) ) )
\end{align*}
Thus using definition of $f$ and $h$, we have
\begin{align*}
    f(W,x_i) =  a^\top h_{i,L}, ~~~ \in \R, ~~~ \forall i \in [n]
\end{align*}

Given $n$ input data points $(x_1 , y_1), (x_2 , y_2) , \cdots (x_n, y_n) \in \R^{d} \times \R$. We define the objective function $\mathcal{L}$ as follows
\begin{align*}
\mathcal{L} (W) = \frac{1}{2} \sum_{i=1}^n ( y_i - f (W,x_i) )^2 .
\end{align*}
 

We can compute the gradient of ${\cal L}$ in terms of $W_{\ell} \in \R^{m_{\ell} \times m_{\ell-1}}$, for all $\ell \geq 2$
\begin{align}\label{eq:gradient}
\frac{\partial\mathcal{L}(W)}{\partial W_{\ell}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, \ell}}_{ m_{\ell} \times m_{\ell} } \left( \prod_{k = \ell+1}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{h_{i, \ell -1}^{\top}}_{1 \times m_{\ell-1}}
\end{align}
Note that the gradient for $W_1 \in \R^{m_1 \times m_0}$ (recall that $m_0 = d$) is slightly different and can not be written by general form. Here is the form
\begin{align}
    \frac{\partial\mathcal{L}(W)}{\partial W_{1}} = \sum_{i = 1}^{n} ( f(W, x_i) - y_i) \underbrace{D_{i, 1}}_{ m_1 \times m_1 } \left( \prod_{k = 2}^{L} \underbrace{W_{k}^{\top}}_{m_{k-1} \times m_k}\underbrace{D_{i, k}}_{ m_{k} \times m_k } \right)  \underbrace{a}_{ m_L \times 1} \underbrace{x_{i}^{\top}}_{1 \times m_{0}}
\end{align}
